Multiple-bounce Smith Microfacet BRDFs using the Invariance Principle

Smith microfacet models are widely used in computer graphics to represent materials. Traditional microfacet models do not consider the multiple bounces on microgeometries, leading to visible energy missing, especially on rough surfaces. Later, as the equivalence between the microfacets and volume has been revealed, random walk solutions have been proposed to introduce multiple bounces, but at the cost of high variance. Recently, the position-free property has been introduced into the multiple-bounce model, resulting in much less noise, but also bias or a complex derivation. In this paper, we propose a simple way to derive the multiple-bounce Smith microfacet bidirectional reflectance distribution functions (BRDFs) using the invariance principle. At the core of our model is a shadowing-masking function for a path consisting of direction collections, rather than separated bounces. Our model ensures unbiasedness and can produce less noise compared to the previous work with equal time, thanks to the simple formulation. Furthermore, we also propose a novel probability density function (PDF) for BRDF multiple importance sampling, which has a better match with the multiple-bounce BRDFs, producing less noise than previous naive approximations.

==> pseudocode.tex <==
% \newcommand{\mycommfont}[1]{\small\texttt{\textcolor[HTML]{4D8F33}{#1}}}
% \SetCommentSty{mycommfont}

% We show pseudo-code of segment term evaluation in Algorithm \ref{alg:SegmentTerm}, BRDF evaluation in Algorithm \ref{alg:eval} and sample in Algorithm \ref{alg:sample}.

% \newpage

% \begin{algorithm}
% \caption{SegmentTerm}
% \label{alg:SegmentTerm}
% \Class(\tcp*[h]{Initialize $\Lambda_o$}){$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     \Def{$m \gets 1$} \;
%     \Def{$N \gets 0$} \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf(\tcp*[h]{Downwards}){$\Lambda_k < 0$} {
%         $N \gets N+1$\;
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\Comment{cache the results when sampled rays are only downwards}
%         }(\tcp*[h]{Upwards}){
        
%             \eIf{$m = 0$}{
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }(\tcp*[h]{Initialize g}){
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }

%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{

%         \If(\tcp*[h]{Return results if cached}){$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }
%         \KwRet{ s }\;
    
%     }
% }

% \end{algorithm}


% \begin{algorithm}
% \caption{Eval}
% \label{alg:eval}
% \Fn{$\mathrm{eval}(\omega_i,\omega_o)$}{
% $\mathrm{SegmentTerm} \  s(\Lambda(\omega_o))$\Comment{ initializing }
% $f \gets 0$\Comment{result}
% $k \gets 0$ \Comment{bounce}
% $w \gets 1$\Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%     $s.\mathrm{addBounce}(\Lambda(\bd_{k}))$\;
%     $k \gets k + 1$\;
%     \If{$k >= rrDepth$}{
%         \If{$\mathrm{rand}()>q$}{
%         break;
%         }
%     $w \gets {w \over q}$\Comment{russian roulette}
%     }
%     $f \gets f + w \cdot v(\bd_{k},\omega_o)\cdot s.\mathrm{getS_k}() $\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
%     ($\bd_{k+1}$,$p_k$) $ \gets $ sample($ \bd_{k} $)\;
%     $w \gets {w \cdot v(\bd_{k},\bd_{k+1}) \over p_k}$\;
% }
%         \KwRet{ f }\;
% }
% \end{algorithm}

% \begin{algorithm}
% \caption{Sample}
% \label{alg:sample}
% \KwResult{weight $w$ and direction $\bd_k$}
% \BlankLine
% $p \gets 1$  \Comment{pdf}
% $k \gets 0$  \Comment{bounce}
% $w \gets 1$  \Comment{weight}
% $\bd_0 \gets -\omega_i$\;
% \While{$\mathrm{true}$}{
%    ($\bd_k$,$p_k$,$w_k$) $ \gets $ sample($ \bd_{k-1} $)\;
%    $w \gets w \cdot w_k$\;
%    $p \gets p \cdot p_k$\;
%     \If{$\bd_k.z > 0$}{
%     $G_1 \gets \frac{1}{|\Lambda(\bd_k)|}$\;
%         \eIf(\tcp*[h]{the ray continues the tracing with $G_1$ as the probablity}){$\mathrm{rand()}<G_1$}
%         {
%             $p \gets p \cdot G_1$\;
%             break;
%         }{
%             $p \gets p \cdot (1-G_1)$\;
%         }
%     }
% $k \gets k+1$\;
%     \If{$k \ge maxBounce$}{
%         break;
%     }
% }
%    $w \gets w \cdot S_k(\bd_0,...,\bd_k)$\;
%    $w \gets {w \over p}$\;
% \end{algorithm}

% \newcommand{\mybox}[3]{
% \begin{tcolorbox}[arc = 0pt, outer arc = 0pt,
%     colback = #1!10!white, colframe = #1!70!black,
%     boxsep = 0pt, left = 2pt, right = 2pt, top = 2pt, bottom = 2pt,
%     boxrule = 0pt, bottomrule = 1pt, toprule = 1pt,width=#2]
% #3
% \end{tcolorbox}
% }

% \newpage

% \begin{algorithm}[h]
% \caption{SegmentTerm}
% \label{alg:coloredST}
% \Class{$\mathrm{SegmentTerm}(\Lambda_o)$} {

%     $N \gets 0$ \;
%     $m \gets 1$ \;
%     \Def{$e[], g[], l[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%        \eIf{$\Lambda_k < 0$} {
%       \mybox{green}{24mm}{
%        % \begin{mybox}[width=30mm]
%        $N \gets N+1$\;
%         % \end{mybox}
%         $l[N] \gets |\Lambda_k|$\;
%         $e[N] \gets \frac{1}{\Lambda_o+|\Lambda_k|}$\;
%         $g[N] \gets 0$\;
%         $m \gets m \cdot e[N]$\;
%         }
%         }{
        
%     \mybox{yellow}{33.5mm}{
%             \eIf{$m = 0$}
%             {
%                $g[N] \gets \frac{g[N]}{\Lambda_k + l[N]}$\;
%         }{
%                $g[N] \gets \frac{1}{\Lambda_k + l[N]}$\;
%                $m \gets 0$\;
%             }
% \mybox{red}{32mm}{
%             \For{$i \gets N-1 ... 1$}{
%                 $g[i] \gets \frac{g[i] + g[i + 1]}{\Lambda_k + l[i]}$\;
%             }}
%             }
%         }
%     }

%     \Fn{$\mathrm{getS_k}()$}{
%     \mybox{cyan}{33.5mm}{
%         \If{$m \ne 0$}{
%         \KwRet{ m }\;
%         }
%          $s \gets 0$\;
         
% \mybox{red}{32mm}{
%         \For{$i \gets N ... 1$}{
%             $s \gets e[i] \cdot (s + g[i])$\;
%         }}
%         \KwRet{ s }\;
%     }
%     }
% }

% \end{algorithm}

% \begin{algorithm}[h]
% \caption{HeightDistribution}
% \label{alg:coloredHD}
% \Class{$\mathrm{HeightDistribution(\Lambda_o)}$} {

%     \Def{$N, a[], b[]$} \;

%     \Fn{$\mathrm{addBounce}(\Lambda_k)$}{
%     \uIf{$N=0$}{
%     $a[1] \gets \Lambda_k$\;
%     $b[1] \gets \Lambda_k$\;
%     $N \gets N+1$\;
%     }
%     \uElseIf{$\Lambda_k < 0$} {
%     \mybox{green}{41.5mm}{
%     \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k-b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         \mybox{red}{40mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[N+1] \gets a[N+1]-a[i] $\;
%         }
%         }
%         $b[N+1] \gets \Lambda_k$\;
%         $N \gets N+1$\;
%     }
%     }
%     \Else{
%     \mybox{yellow}{33.5mm}{
%     \mybox{red}{32mm}{
%         \For{$i \gets 1 ... N$}{
%             $a[i] \gets a[i]\frac{\Lambda_k}{\Lambda_k+b[i]} $\;
%         }
%         }
%         $a[N+1] \gets 0$\;
%         $b[N+1] \gets -\Lambda_k$\;}
%     }
% }
%     \Fn{$\mathrm{getP_{exit}}()$}{
%     \mybox{cyan}{28.5mm}{
%          $s \gets 0$\;
%     \mybox{red}{27mm}{
%         \For{$i \gets 1 ... N$}{
%             $s \gets s + \frac{a[i]}{\Lambda_o+b[i]}$\;
%         }
%         }
%         \KwRet{ s }\;
%         }
    
%     }
% }

% \end{algorithm}

==> sec_method.tex <==


\section{Path integral of multiple-bounce BSDF}

\myfigure{z}{z.png}{Notations. From Bitterli et al. Redraw latter.}

We follow the conclusion from Dupuy et al.~\shortcite{Dupuy:2016:Unification}, that the microfacet model is equivalent to a semi-homogeneous media. As shown in Fig.~\ref{fig:z}, the range of the media is $(-\infty,0]$. 

We first define a path which is the same as in the media, which includes directions and distances. For example, a path with length $k$ is defined as: $(\bd_0, \bt_0, \bd_1, \bt_1, \cdots, \bd_{k-1}, \bt_{k-1}, \bd_{k})$, where $\bd_0 = \omega_i$ and $\bd_k = \omega_o$. All the paths with end directions as $\omega_i$ and $\omega_o$ form a path space. The multiple scattering of $\omega_i$ and $\omega_o$ consists of the contribution of this entire path space. 

The multiple scattering in a microfacet model is equivalent to the multiple scattering within the media. The contribution of each path includes two components: vertex term which serves as the phase function in the media, and a segment term which is equivalent to the attenuation along the path.

\added{The free-flight probability density function is missing here.}

Thus, the contribution of all the paths with length $k$ is:
\begin{equation}
    \rho_k(\omega_i, \omega_o) = \int_{\mathcal{P}} \left (\prod_{i=0}^{i=k-1}v_i(\bd_i,\bd_{i+1}) \right)  \left (\prod_{i=0}^{i=k-1}Tr(\bt_i,\bd_i) \right) \dd \mu(\overline{\bt},\overline{\bd}),
    \label{eq:integral}
\end{equation}
where $v_i$ is the vertex term, including the Fresnel term, normal distribution function and the Jacobian term along the path, which is the same as in Wang's model, as shown in Eqn.~\ref{eq:v_r}. The vertex term is independent of the distance along the path. $Tr$ is the attenuation of a segment with direction $\bd_i$ and distance $\bt_i$ along the path in the media. $Tr(\bt_i,\bd_i)$ is defined as
\begin{equation}
    Tr(\bt_i,\bd_i) = e^{-(\bt_i)\sigma(\bd_i)}.
    \label{eq:T}
\end{equation}
$\mathcal{P}$ represents the path space, and $\dd \mu(\overline{\bt},\overline{\bd}) = \dd \overline{\bt} \cdot \dd \overline{\bd}$ is the product of standard Lebesgue measures of the distance $\overline{\bt} = \bt_0, \cdots, \bt_{k-1}$ and the solid angle measures of the directions $\overline{d} = \bd_0, \cdots, \bd_{k}$. 


Starting from Eqn.~\ref{eq:integral}, the vertex terms can be moved outside the distance measurement, resulting in 
\begin{equation}
    \rho_k(\omega_i, \omega_o) = \int_{\Omega} \left (\prod_{i=0}^{i=k-1}v_i(\bd_i,\bd_{i+1}) \right)  \int_{\mathcal{T}} \left (\prod_{i=0}^{i=k-1}Tr(\bt_i,\bd_i) \right) \dd \mu(\overline{\bt}) \dd \mu(\overline{\bd}),
    \label{eq:integralV_S}
\end{equation}


\paragraph{Discussion.} Wang et al.~\shortcite{wang2021positionfree} proposed two ways to compute the segment term: a height-uncorrelated and height-correlated version. Both of them are independent of the distance or the height. Different from Wang's model, we relax this independent-bounce assumption and solve this segment term for the entire path directly. 

\added{The deviation of the above equation is similar to Bitterli et al. But we need them. What's the difference between ours and Bitterli et al.}
 %For each sampled path, the path contribution is computed by accumulating the vertex terms and segment terms along the path. The main difference between our model and Wang's model is that the shadowing-masking function is computed the entire path directly, rather than for each segment separately. In this case, we actually do not use the position-free assumption in Wang's model.

\subsection{Path shadowing-masking function}

Similar to both Wang et al.~\shortcite{wang2021positionfree} and Bitterli et al.~\shortcite{BitterliAndd'Eon:2022}, the computation of the outer integral in Eqn.~\ref{eq:integralV_S} requires Monte Carlo sampling. The direction path space defined by an incoming and outgoing direction pair is sampled by an unidirectional or bidirectional sampler. So in this paper, we focus on the inner integral, which is given a directional path: $(\bd_0, \bd_1,  \cdots, \bd_{k-1}, \bd_{k})$, how to compute its segment term or shadowing-masking function. The shadowing-masking function is defined as the integral of the distance space.
\added{Here we have two spaces. Do we need to define them explicitly?}

The key equation to be solved is shown here:
\begin{equation}
    S_k(\bd_0,\cdots, \bd_k) =  \int_{\mathcal{T}} \left (\prod_{i=0}^{i=k}Tr(\bt_i,\bd_i) \right) \dd \mu(\overline{\bt}),
    \label{segmentIntegral}
\end{equation}

Note that, using Monte Carlo sampling could solve Eqn.~\ref{segmentIntegral}. But, in this paper, we solve this equation analytically and also prove that the multiple-bounce shadowing-masking function is independent of the distance / height, resulting in a \emph{height-free} model. This is the key point of our paper.

\subsection{Changing integral variable}

Before we deriving the solution for Eqn.~\ref{segmentIntegral}, we first change the integral variable. Different from Bitterli et al.~\shortcite{BitterliAndd'Eon:2022}, we change the variable from distance to the uniform random variant, which allowing for performing integral along the depth. 

The media can be parameterized with a uniform random domain $\mathcal{U}$, where the mapping between the uniform random domain and the height is as follows: $h = \mathrm{log} (u) $, where $u$ is a random uniform variate defined on $[0, 1]$. More details can be found in Dupuy et al.~\shortcite{Dupuy:2016:Unification}. Since $u$ is uniformly defined in the $\mathcal{U}$ space, it makes the integral much simpler. For path with length $k$, the path's format with $u$ is defined as $(u_0,\bd_0,\cdots,\bd_k,u_{k+1})$, where $u_0 = \infty$ $u_{k+1} = \infty$. This formulation is actually equivalent to the distance formation.


%We further change the variable of in the integral from the height difference to the uniform variable $u$, since $u$ is uniformly defined in the $\mathcal{U}$ space, which makes the integral much simpler.

\begin{equation}
    S_k(\bd_0, \cdots, \bd_k) =  \int_{\mathcal{U}} \left (\prod_{i=0}^{i=k}Tr^{z}(\mathrm{log}(u_i), \mathrm{log}(u_{i+1}),\bd_i) \right) \dd u,
    \label{eq:segmentIntegral_U}
\end{equation}
where $Tr^{z}$ is
\begin{equation}
    Tr^z(h_i,h_{i+1},\bd_i) = e^{-|h_{i+1} - h_{i}|a_i},
    \label{eq:TrU}
\end{equation}
and $a_i$ is defined as:
\begin{equation}
    a_i(\bd_i) =\frac{\sigma(\bd_i)}{|(\bd_i)_z|},
\end{equation}
where $(\bd_i)_z$ is the $z$ component of $\bd_i$ and $h_i = \mathrm{log} (u_i)$.

%    T(h_i,h_j, d_i) = e^{-(h_i-h_j)a_1},
%    \label{eq:T}
%\end{equation}
%and $a_i$ is defined as:
%\begin{equation}
%    a_i = \frac{\sigma(d_i)}{\mathrm{cos \theta_i}}
%\end{equation}.

\added{We need to check the change of the variable is written in the correct way!!}

We will derive the analytical solution to Eqn.~\ref{eq:segmentIntegral_U} in the next section. We only consider the reflective microfacet for now, and leave the refractive microfacet for the future work.

\section{Shadowing-masking function for a multi-bounce reflective path}

In the following sections, we will show how derive the formation of our path shadowing-masking function for the two-bounce case first, and then we extend it to three bounces. In the end, the formulation for arbitrary bounces are derived.

\subsection{Path shadowing-masking function for two-bounce case}

\myfigure{twobounce}{twoBounce.jpg}{The configuration of the two-bounce case.}

Consider the two-bounce case with $\omega_i = -\bd_0$ and $\omega_o = \bd_2$, as shown in Fig.~\ref{fig:twobounce}. Assume that we already have the second direction $\bd_1$, so we have a path consisting of directions: $p = (\bd_0, \bd_1, \bd_2)$.

%Let's assume that we have a height distribution underlying. Thus, the path $p = d_1, d_2, d_3$ is not a single path, but is a path space, as the height at $v_1$ and $v_2$ are not fixed. If we set the height at $v_1$ as $h_1$ and the height at $v_2$ as $h_2$. The shadowing-masking function or the attenuation along this path is computed as:
%\begin{equation}
%s_h(d_1,h_1,d_2,h_2,d_3) = T(h_1, +\infty, d_1)  T(h_1, h_2, d_2)  T(h_2, +\infty, d_3),
%    \label{eq:twobouncePathH}
%\end{equation}
%where $T(h_i, h_j, d_i)$ is the attenuation function from height $h_i$ to $h_j$ with direction $d_i$ defined as
%\begin{equation}
%    T(h_i,h_j, d_i) = e^{-(h_i-h_j)a_1},
%    \label{eq:T}
%\end{equation}
%and $a_i$ is defined as:
%\begin{equation}
%    a_i = \frac{\sigma(d_i)}{\mathrm{cos \theta_i}}
%\end{equation}.

%We integrate the shadowing-masking function over the heights along the path. Here we transform the integration variable from height to the random uniform variate:
Eqn.~\ref{eq:segmentIntegral_U} for the two-bounce case is:
\begin{equation}
\begin{aligned}
        &S_{\mathrm{R}^2}(\bd_0, \bd_1, \bd_2) = \int_{u_1 = 0}^{u_1 = 1} Tr^z(\mathrm{log}(u_1), +\infty, \bd_0)\\
       & \int_{u_2 = u1}^{u_2 = 1}Tr^z(\mathrm{log}(u_1), \mathrm{log}(u_2), \bd_1)  Tr^z(\mathrm{log}(u_2), +\infty, \bd_2) \dd u_1 \dd u_2. 
\end{aligned}
    \label{eq:twobouncePath}
\end{equation}
Note that the range of $u_2$ is determined by the direction of $\bd_1$. If $\bd_1$ points to the upper hemisphere, the range of $u_2$ will be $(u_1, 1)$, otherwise the range will be $(0,u_1)$. Let's assume $\bd_1$ points to the lower hemisphere first.

By expanding the $Tr^{z}$ with Eqn.~\ref{eq:T}, we get a closed-form formula:
\begin{equation}
    S_{\mathrm{R}^2}(\bd_0, \bd_1, \bd_2| \bd_1.z < 0) = \frac{1}{(\Lambda(\bd_1) + \Lambda(\bd_2) + 1)(\Lambda(\bd_0) + \Lambda(\bd_2) + 2)}. 
    \label{eq:twobouncePath}
\end{equation}
The derivation details are shown in the Appendix.

Similarly, when $\bd_1$ points to the upper hemisphere, we get the following formula:
\begin{equation}
    S_{\mathrm{R}^2}(\bd_0, \bd_1,\bd_2 | \bd_1.z > 0) = \frac{1}{(\Lambda(\bd_0) + \Lambda(\bd_1) + 1)(\Lambda(\bd_0) + \Lambda(\bd_2) + 2)}. 
    \label{eq:twobouncePath}
\end{equation}

The formulation of two-bounce case are:
\begin{equation}
	S_{\mathrm{R}^2}(\bd_0,\bd_1,\bd_2) = \left\{
	\begin{array}{lr} 
	     \frac{1}{(\Lambda(\bd_1) + \Lambda(\bd_2) + 1)(\Lambda(\bd_0) + \Lambda(\bd_2) + 2)}, \mathrm{~~if~~} \bd_1.z < 0, \\
	      \frac{1}{(\Lambda(\bd_0) + \Lambda(\bd_1) + 1)(\Lambda(\bd_0) + \Lambda(\bd_2) + 2)}, \mathrm{~~if~~} \bd_1.z > 0.
    \end{array}  
	\right.
	\label{eq:threeBounce}
\end{equation}

Now, we get a closed-formulation for the shadowing-masking function of a path with two bounces. 


\subsection{Path shadowing-masking function for three-bounce case.}

The extension from the two-bounce case to the general case is not straightforward, since there more case which is not shown in the two-bounce case. Therefore, we derive the formation for the three-bounce in this section, and then show the general case in the next section.

\myfigure{threeBounce}{threebounce.jpg}{The configuration of the three-bounce case.}

The configuration of the paths with three bounces include three cases, as shown in Fig.~\ref{fig:threeBounce}. The derivation of the first and the second case is similar to the two-bounce case, so we leave the derivation in the supplementary, and focus on the third case.

The main difficulty comes from the relative height between $u_1$ and $u_3$. We need to know the integration range of $h_3$. If $h_3 > h_1$, the integral range of $h_3$ will be $(u_1, 1)$, otherwise the integral range will be $(u_2, u_1)$. These cases need to be considered separately, and the final contribution of the third case two be the sum of these two cases. 

If $h_3 > h_1$, the shadowing-masking function of the path $(\bd_0,\cdots,\bd_3)$ is:
\begin{equation}
    \begin{aligned}
           &S_{\mathrm{R}^3}(\bd_0,\cdots,\bd_3 | \bd_1.z < 0 \& \bd_2.z > 0 \& h_3 > h_1) = \\ &\frac{1}{(\Lambda(\bd_1)+\Lambda(\bd_2)+1)
           (\Lambda(\bd_0)+\Lambda(\bd_2)+2)(\Lambda(\bd_0)+\Lambda(\bd_3)+3)}.
    \end{aligned}
    \label{eq:threeBounce_case3_1}
\end{equation}


If $h_3 < h_1$, the shadowing-masking function of the path $(\bd_0,\cdots,\bd_3)$ is:
\begin{equation}
    \begin{aligned}
           &S_{\mathrm{R}^3}(\bd_1,\cdots,\bd_3 | \bd_1.z < 0 \& \bd_2.z > 0 \& h_3 < h_1) = \\
           &\frac{1}{(\Lambda(\bd_1)+\Lambda(\bd_2)+1)
           (\Lambda(\bd_1)+\Lambda(\bd_3)+2)(\Lambda(\bd_0)+\Lambda(\bd_3)+3)}.
    \end{aligned}
    \label{eq:threeBounce_case3_2}
\end{equation}

By merging Eqn.~\ref{eq:threeBounce_case3_1} and Eqn.~\ref{eq:threeBounce_case3_2}, we get the formulation:
\begin{equation}
    \begin{aligned}
           &S_{\mathrm{R}^3}(\bd_0,\cdots,\bd_3 | \bd_1.z < 0 \& \bd_2.z > 0) = \\ &\frac{1}{(\Lambda(\bd_1)+\Lambda(\bd_2)+1)(\Lambda(\bd_0)+\Lambda(\bd_3)+3)} \\
&\left ( \frac{1}{\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{2}\right)+2}+\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)+\Lambda\left(\mathbf{d}_{3}\right)+2} \right ).
    \end{aligned}
    \label{eq:threeBounce_case3}
\end{equation}

The formulation of all the cases are:
\begin{equation}
S_{\mathrm{R}^3}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\begin{cases}{\Tiny\enspace\space}\frac{1}{\left(\Lambda\left(\mathbf{d}_{1}\right)+\Lambda\left(\mathbf{d}_{2}\right)+1\right)\left(\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{3}\right)+3\right)} \\
\left ( \frac{1}{\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{2}\right)+2}+\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)+\Lambda\left(\mathbf{d}_{3}\right)+2} \right )  , \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0, \\
\frac{1}{\left(\Lambda\left(\mathbf{d}_{2}\right)+\Lambda\left(\mathbf{d}_{3}\right)+1\right)\left(\Lambda\left(\mathbf{d}_{1}\right)+\Lambda\left(\mathbf{d}_{3}\right)+2\right)\left(\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{3}\right)+3\right)}, \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 ,\\
\frac{1}{\left(\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{1}\right)+1\right)\left(\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{2}\right)+2\right)\left(\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{3}\right)+3\right)}, \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0.
\end{cases}
	\label{eq:threeBounce}
\end{equation}


\subsection{Path shadowing-masking function for arbitrary bounces.}

Most of the cases have been covered by the two-bounce and the three-bounce cases. Now, let's derive the general case in this section. 

Before deriving the formulation, there is one important observation. There is only one vertex $v_i$ along a path with bounce $k$: $(\bd_0,\bd_1,\cdots,\bd_{k})$, which satisfy the following requirements: $\bd_{i+1}.z > 0$ and $\bd_i.z < 0$. We call this vertex \emph{corner} vertex.

If this corner vertex is the first or last vertex along the path, then the derivation of the shadowing-masking function of the path is simple: 
\begin{equation}
           S_{\mathrm{R}^k}(\bd_0,\cdots,\bd_{k}) = 
           	\begin{cases}
            \frac{S_{\mathrm{R}^{ k-1}}(\bd_0,\cdots,\bd_{k-1})}{\Lambda(\bd_0) + \Lambda(\bd_{k}) + k},\mathrm{~~if~~} \bd_1.z > 0~~ \mathrm{and} ~~\bd_{k-1}.z > 0, \\
             \frac{S_{\mathrm{R}^{k-1}}(\bd_1,\cdots,\bd_{k})}{(\Lambda\bd_0) + \Lambda(\bd_{k}) + k},\mathrm{~~if~~} \bd_1.z < 0~~ \mathrm{and} ~~\bd_{k-1}.z < 0. \\
            \end{cases}  
    \label{eq:general}
\end{equation}

If the corner vertex is not either the first nor the last vertex, then the  the shadowing-masking function is computed by the following formulation:
\begin{equation}
     \begin{aligned}
           S_{\mathrm{R}^k}(\bd_0,\cdots,\bd_{k}) = \frac{S_{\mathrm{R}^{k-1}}(\bd_0,\cdots,\bd_{k-1}) + S_{\mathrm{R}^{k-1}}(\bd_1,\cdots,\bd_{k})}{\Lambda(\bd_0) + \Lambda(\bd_{a}) + k}.
     \end{aligned}
    \label{eq:general}
\end{equation}

\added{Do we need to proof this?}

\section{Shadowing-masking function for a multi-bounce refractive path}

The method in Bitterli et al.~\shortcite{BitterliAndd'Eon:2022} cannot be used to calculate a refractive path, but this does not mean that the refraction is dependent to the height distribution. In this section, we proved that the dielectric microfacet is still unrelated to the height distribution.

\subsection{Essential mathematics definitions}
To solve this problem, we need to introduce some new formulas. Most of them are common in mathematics and theoretical physics, but those are new concepts for computer graphics.

Gauss~\shortcite{gauss1812} introduced the hypergeometric function ${_{2}F_{1}}$ , and Pochhammer~\shortcite{pochhammer1870} promoted it to the generalized hypergeometric functions ${_{p}F_{q}}$. These functions are defined by infinite series:
\begin{equation}
     \begin{aligned}
     {_{p}F_{q}}\left(a_1,a_2,\cdots,a_p;b_1,b_2,\cdots,b_q,z\right)=\sum_{k=0}^{\infty}\frac{{\Tiny\displaystyle\prod_{i=1}^{p}} \frac{\Gamma \left ( a_i+k\right)}{\Gamma\left(a_i\right)}}{{\Tiny\displaystyle\prod_{j=1}^{q}}\frac{\Gamma \left ( b_j +k\right ) }{\Gamma \left ( b_j\right )}}\frac{z^k}{k!}
     \end{aligned}
    \label{eq:hypergeometric}
\end{equation}
Where $\Gamma$ is the Gamma function, which is the analytical continuation of $(x-1)!$.

A height-correlated analytical $S_{\mathrm{T}}$ term for a single refractive scattering is given in \cite{Pinel:05}, where the Beta function is used:

\begin{equation}
     \begin{aligned}
    \mathrm{B}(a, b)=\int_{0}^{1} t^{a-1}(1-t)^{b-1} \mathrm{~d}t
     \end{aligned}
    \label{eq:beta}
\end{equation}

These functions are related as:
\begin{equation}
     \begin{aligned}
    \mathrm{B}(a, b)=\frac{\Gamma(a)\Gamma(b)}{\Gamma(a+b)}=\frac{z^a}{a}{_{2}F_{1}}(a,1-b;1+a,z)
     \end{aligned}
\end{equation}

When we tried to solve the refraction problems, we found that the existing mathematical functions could not meet our needs, we needed to define some new functions, which we called  \emph{generalized beta functions}:
\begin{equation}
     \begin{aligned}
 &\mathrm{B}^k(a_1,a_2,\cdots,a_k;b_1,b_2,\cdots,b_k)=\\ &\int_{\displaystyle [0,1]\times \prod_{m=1}^{k-1}[0,\mathcal{U}_m ] }\prod_{n=1}^{k} \mathcal{U}_n^{a_n-1}(1-\mathcal{U}_n)^{b_n-1}\mathrm{~d}\overline{\mathcal{U}}
     \end{aligned}
    \label{eq:generalizedbeta}
\end{equation}
Where $\mathrm{B}^1(a_1;b_1)=\mathrm{B}(a_1,b_1)$.

We will prove an important conclusion in appendix:
\begin{equation}
     \begin{aligned}
&\mathrm{B}^2(a_1,a_2;b_1,b_2)= \\
&\frac{1}{a_2}\mathrm{B}\left ( a_1+a_2,b_1 \right ) {{_3}F{_2}}\left ( a_2,1-b_2,a_1+a_2;a_2+1,a_1+a_2+b_1,1 \right )
     \end{aligned}
    \label{eq:beta2}
\end{equation}
\subsection{Path shadowing-masking function for two-bounce case}
\begin{equation}
     \begin{aligned}
     S_{\small\mathrm{TR}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=
\begin{cases}
\frac{\mathrm{B}(\Lambda\left(\mathbf{d}_{1}\right)+1,\Lambda\left(\mathbf{d}_{0}\right)+1)-\mathrm{B}(\Lambda\left(\mathbf{d}_{2}\right)+2,\Lambda\left(\mathbf{d}_{0}\right)+1) }{\left(\Lambda\left(\mathbf{d}_{2}\right)-\Lambda\left(\mathbf{d}_{1}\right)+1\right)},\\
\text { if } \mathbf{d}_{1} . z<0 \\
\frac{\mathrm{B}(\Lambda\left(\mathbf{d}_{2}\right)+2,\Lambda\left(\mathbf{d}_{0}\right)+1) }{\left(\Lambda\left(\mathbf{d}_{2}\right)+\Lambda\left(\mathbf{d}_{1}\right)+1\right)}, \text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     S_{\small\mathrm{RT}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=
\begin{cases}
\frac{\mathrm{B}(\Lambda\left(\mathbf{d}_{1}\right)+1,\Lambda\left(\mathbf{d}_{2}\right)+1)-\mathrm{B}(\Lambda\left(\mathbf{d}_{0}\right)+2,\Lambda\left(\mathbf{d}_{2}\right)+1) }{\left(\Lambda\left(\mathbf{d}_{0}\right)-\Lambda\left(\mathbf{d}_{1}\right)+1\right)},\\
\text { if } \mathbf{d}_{1} . z<0 \\
\frac{\mathrm{B}(\Lambda\left(\mathbf{d}_{0}\right)+2,\Lambda\left(\mathbf{d}_{2}\right)+1) }{\left(\Lambda\left(\mathbf{d}_{0}\right)+\Lambda\left(\mathbf{d}_{1}\right)+1\right)}, \text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     S_{\small\mathrm{TT}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=
\begin{cases}
\mathrm{B}^2(1-\Lambda\left(\mathbf{d}_{1}\right),1+\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{2}\right)+1,\Lambda\left(\mathbf{d}_{0}\right)+1), \\
\text { if } \mathbf{d}_{1} . z<0 \\
\mathrm{B}^2(1-\Lambda\left(\mathbf{d}_{1}\right),1+\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{0}\right)+1,\Lambda\left(\mathbf{d}_{2}\right)+1), \\
\text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}
\subsection{Path shadowing-masking function for three-bounce case}
\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{TRR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{1}{\Lambda(\mathbf{d}_3)-\Lambda(\mathbf{d}_2)+1}\\
\left ( \frac{\mathrm{B}(2+\Lambda(\mathbf{d}_2),1+\Lambda(\mathbf{d}_0))}{\Lambda(\mathbf{d}_1)+\Lambda(\mathbf{d}_2)+1}-\frac{\mathrm{B}(2+\Lambda(\mathbf{d}_3),1+\Lambda(\mathbf{d}_0))}{\Lambda(\mathbf{d}_1)+\Lambda(\mathbf{d}_3)+2} \right )  \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0 \\
\frac{\mathrm{B}(1+\Lambda(\mathbf{d}_1),1+\Lambda(\mathbf{d}_0))-\mathrm{B}(2+\Lambda(\mathbf{d}_3),1+\Lambda(\mathbf{d}_0))}{(\Lambda(\mathbf{d}_3)-\Lambda(\mathbf{d}_1)+2)(\Lambda(\mathbf{d}_3)+\Lambda(\mathbf{d}_2)+1)}\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0 \\
\frac{1}{\Lambda(\mathbf{d}_3)-\Lambda(\mathbf{d}_2)+1}\\
\left ( \frac{\mathrm{B}(1+\Lambda(\mathbf{d}_1),1+\Lambda(\mathbf{d}_0))-\mathrm{B}(2+\Lambda(\mathbf{d}_2),1+\Lambda(\mathbf{d}_0))}{\Lambda(\mathbf{d}_2)-\Lambda(\mathbf{d}_1)+1}-\right.\\
\left.\frac{\mathrm{B}(1+\Lambda(\mathbf{d}_1),1+\Lambda(\mathbf{d}_0))-\mathrm{B}(3+\Lambda(\mathbf{d}_3),1+\Lambda(\mathbf{d}_0))}{\Lambda(\mathbf{d}_3)-\Lambda(\mathbf{d}_1)+2} \right )  \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 \\
\frac{\mathrm{B}(3+\Lambda(\mathbf{d}_3),1+\Lambda(\mathbf{d}_0))}{(\Lambda(\mathbf{d}_3)+\Lambda(\mathbf{d}_2)+1)(\Lambda(\mathbf{d}_1)+\Lambda(\mathbf{d}_3)+2)}\\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{RTR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0 \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0 \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{RRT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0 \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0 \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{TTR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0 \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0 \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{TRT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{1}{\Lambda (\mathbf{d}_2)+\Lambda (\mathbf{d}_1)+1}\bigg(\mathrm{B}(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_3))\mathrm{B}(2+\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_0))-\\
\Big(\mathrm{B}^2(2+\Lambda (\mathbf{d}_2),1-\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))-\\
\mathrm{B}^2(2+\Lambda (\mathbf{d}_2),2+\Lambda (\mathbf{d}_1);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))\Big )\bigg )\normalsize, \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0 \\
\frac{1}{1-\Lambda (\mathbf{d}_2)-\Lambda (\mathbf{d}_1)}\bigg(\mathrm{B}(1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_0))\Big(\mathrm{B}(1+\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_3))-\\
\mathrm{B}(2-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))\Big )-\Big (\mathrm{B}^2(2-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0)\\
,1+\Lambda (\mathbf{d}_3))-\mathrm{B}^2(2-\Lambda (\mathbf{d}_2),2-\Lambda (\mathbf{d}_1);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))\Big )\bigg)\normalsize,\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0 \\
\frac{1}{\Lambda (\mathbf{d}_2)-\Lambda (\mathbf{d}_1)+1}\bigg(\mathrm{B}(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_3))\Big(\mathrm{B}(2-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))-\\
\mathrm{B}(2+\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_0))\Big )-\Big (\mathrm{B}^2(2+\Lambda (\mathbf{d}_1),1-\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0)\\
,1+\Lambda (\mathbf{d}_3))-\mathrm{B}^2(2+\Lambda (\mathbf{d}_2),2-\Lambda (\mathbf{d}_1);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))\Big )\bigg),\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 \\
\frac{1}{\Lambda (\mathbf{d}_2)-\Lambda (\mathbf{d}_1)+1}
\left(\mathrm{B}^2(2-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))-\right.\\
\left.\mathrm{B}^2(2-\Lambda (\mathbf{d}_2),2+\Lambda (\mathbf{d}_1);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))\right),\\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{RTT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\mathrm{B}(2+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_2))\mathrm{B}(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_3))-\mathrm{B}^2(1+\Lambda (\mathbf{d}_2),1-\Lambda (\mathbf{d}_2);2+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))}{\Lambda (\mathbf{d}_0)+\Lambda (\mathbf{d}_1)+1}, \\
\text { if } \mathbf{d}_{1}.z>0 \text { and } \mathbf{d}_{2}.z<0 \\
\frac{\mathrm{B}^2(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))-\mathrm{B}^2(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);2+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))}{\Lambda (\mathbf{d}_0)-\Lambda (\mathbf{d}_1)+1}, \\
\text { if } \mathbf{d}_{1}.z<0 \text { and } \mathbf{d}_{2}.z>0 \\
\frac{1}{\Lambda (\mathbf{d}_0)-\Lambda (\mathbf{d}_1)+1}\scriptsize\bigg(\mathrm{B}(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_3))\Big(\mathrm{B}(1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_2))-\\
\scriptsize\mathrm{B}(2+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_2))\Big )-\Big (\mathrm{B}^2(1+\Lambda (\mathbf{d}_2),1-\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))-\\
\scriptsize \mathrm{B}^2(1+\Lambda (\mathbf{d}_2),1-\Lambda (\mathbf{d}_2);2+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))\Big )\bigg)\normalsize,\\
\text { if } \mathbf{d}_{1}.z<0 \text { and } \mathbf{d}_{2}.z<0 \\
\frac{\mathrm{B}^2(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);2+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_3))}{\Lambda (\mathbf{d}_0)+\Lambda (\mathbf{d}_1)+1},\\
\text { if } \mathbf{d}_{1}.z>0 \text { and } \mathbf{d}_{2}.z>0
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
     &S_{\small\mathrm{TTT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\scriptsize  \mathrm{B}^3(1-\Lambda (\mathbf{d}_1),1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))\normalsize,\\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0 \\
\scriptsize  \mathrm{B}^3(1-\Lambda (\mathbf{d}_2),1-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_1);1+\Lambda (\mathbf{d}_3),1+\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_0))\normalsize,\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0 \\
{\Tiny\enspace} \scriptsize  \mathrm{B}(1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_0))\mathrm{B}^2(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);1-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))-\\
\scriptsize  \mathrm{B}^3(1+\Lambda (\mathbf{d}_1),1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0),1-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))\normalsize,\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0 \\
\scriptsize\mathrm{B}^2(1-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_1))\mathrm{B}(1-\Lambda (\mathbf{d}_2),1+\Lambda (\mathbf{d}_3))-\\
\scriptsize  \mathrm{B}^3(1-\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_2),1-\Lambda (\mathbf{d}_2);1+\Lambda (\mathbf{d}_0),1+\Lambda (\mathbf{d}_1),1+\Lambda (\mathbf{d}_3))\normalsize,\\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0
\end{cases}
     \end{aligned}
\end{equation}
\subsection{Path shadowing-masking function for arbitrary bounces.}

What we can prove is that $S$ with any order of refraction can be expressed as a finite-order composite of generalized beta functions which less than or equal to the order of refraction and elementary functions. But we can also prove that the generalized beta functions of order greater than or equal to 3 cannot be expressed as a finite-order composite of generalized hypergeometric functions, generalized beta functions of order less than 3, and elementary functions.



==> sup_sec_slab.tex <==
\section{Formulation for medium slab}
\label{supsec:slab}
% 对medium slab的推导与论文中对微表面的推导基本一致，考虑厚度为$T$的medium slab，从下方减去一层厚度为$\Delta\tau$的薄层，并加在slab的顶面上，设反射和透射的多重散射相位函数分别为$\rho_r$和$\rho_t$，列出发生改变几种情况即可得到最终的表达式。要注意的是透射还会额外的考虑一个Delta transmission。
The derivation for the medium slab is similar to the derivation for microfacet in the paper. Considering a medium slab with a thickness of $T$, we subtract a thin layer with a thickness of $\Delta\tau$ from the bottom and add it to the top surface of the slab. Let $\rho_r$ and $\rho_t$ represent the multiple scattering phase functions for reflection and transmission, respectively. By considering various cases where changes occur, we can obtain the final expressions. It is important to note that transmission also includes delta transmission.
\subsection{Reflection}
% \textbf{:}
\begin{equation}
\begin{aligned}
&\rho _r\left(\omega_{i}, \omega_{o}\right) = \frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)}\bigg(v\left(\omega_{i}, \omega_{o}\right)+\\
&\int_{\Omega^+}\Big(\rho _r\left(\omega_{i}, \omega\right) v\left(\omega, \omega_{o}\right)+v\left(\omega_{i},-\omega\right) \rho _r\left(-\omega, \omega_{o}\right)\Big) \mathrm{d} \omega \\
&+\int_{\Omega^+} \int_{\Omega^+}\Big(\rho _r\left(\omega_{i}, \omega_{1}\right) v\left(\omega_{1},-\omega_{2}\right)\rho _r\left(-\omega_{2}, \omega_{o}\right)-\\
&\rho _t\left(\omega_{i},-\omega_{1}\right) v\left(-\omega_{1}, \omega_{2}\right) \rho _t\left(-\omega_{2}, -\omega_{o}\right)\Big) \mathrm{d} \omega_{1} \mathrm{~d} \omega_{2}\bigg).
\end{aligned}
\end{equation}
% 透射：
\subsection{Transmission}
% \textbf{Transmission:}

\begin{equation}
\begin{aligned}
&\rho _t\left(\omega_{i}, \omega_{o}\right) = \delta\left(\left\|\omega_{i}-\omega_{o}\right\|\right) e^{-T \Lambda\left(-\omega_{i}\right)}+\frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)}\\
&\bigg(\int_{\Omega^+}\Big(v\left(\omega_{i},-\omega\right) \rho_t\left(-\omega, \omega_{o}\right)-\rho_t\left(\omega_{i},-\omega\right) v\left(-\omega, \omega_{o}\right)\Big) \mathrm{d} \omega \\
&+\int_{\Omega^+} \int_{\Omega^+}\Big(\rho_r\left(\omega_{i}, \omega_{1}\right) v\left(\omega_{1},-\omega_{2}\right)\rho_t\left(-\omega_{2}, \omega_{o}\right)-\\
&\rho_t\left(\omega_{i},-\omega_{1}\right) v\left(-\omega_{1}, \omega_{2}\right) \rho_r\left(-\omega_{2}, -\omega_{o}\right)\Big) \mathrm{d} \omega_{1} \mathrm{~d} \omega_{2}\bigg).
\end{aligned}
\end{equation}

==> temp_method_refraction.tex <==
\subsection{Multi-bounce formulation for the refractive microfacet model}
\label{sec:refraction}

%对于折射，来说，事情变得复杂了起来，我们需要用4组带深度的积分方程来描述其过程：

We also use the variance principle for the refractive surfaces. Different from the reflective surface, there are four combinations considering the inside / outside of the surface and the reflection or refraction interaction. We use $\rho_r^{o}$ and $\rho_r^{i}$ to represent reflection at the outside / inside of the surface respectively. We use $\rho_t^{o}$ to represent the refraction from the outside to the inside of the surface, and $\rho_t^{i}$ for the vice versa.

For each of these four cases, we formulate the changes of the radiance via the invariance principle. The question is how to derive the formulation in the refraction case. In the reflective surface, we model the microfacet model as a homogeneous media and add a layer on top of the media; then we derive the multiple scattering formulation using the invariance principle. However, for the refractive surface, the derivation is not as simple as the reflection case. 

在反射情况下，只用了线性主部，但是在折射中没有办法只用线性主部。为什么？或者说为什么在折射情况下需要在下面去掉一个layer， 而在reflection情况下不需要去掉这个layer。以及去掉这个layer的含义到底是什么。
另外，是如何model的，仍然是medium么还是说用height field。用medium又应该如何解释呢？

So, for the refractive case, we model the media as \added{xxx}. Then add a layer on top of the media and reduce a layer at the bottom. Then we will show how these two layers change the four cases ($\rho_r^o,\rho_r^{i},\rho_t^o,\rho_t^{i}$). We only provide the full derivation of the $\rho_r^{o}$ in the main paper and \added{leave the others in the supplementary.} 

\myfigure{refractionCases}{refractionCases.png}{\added{The first case is missing.} Six cases of $\rho_r^{o}$ due to the adding of the thin layer on a refractive microgeometry. \added{Redraw later.} }

We first consider both the incoming light and the outgoing light locates outside the surface with a reflection interaction. Adding a layer on the top of the medium and reducing a layer at the bottom results in six cases, including the four cases in the reflection. The other two cases are:
\begin{itemize}
    \item one refractive interactions along the incoming ray $\omega_i$, represented as $TT^*$,
    \item one refractive interactions along the outgoing ray $\omega_o$, represented as $T^*T$.
\end{itemize}
Therefore, we have: $R^*, R, RR^*,R^*R, TT^*$, and $T^*T$. Do we only have these six cases? As we talked earlier in the reflection case, we only consider at most one scattering event in the adding layer, since more scattering events are quantities of a higher order of smallness relative to $\Delta \tau$. Besides these six cases, do we have other cases with at most one scattering event in the adding layer? Note that, the current case is about $\rho_r^{o}$, so the entire light transport should be a reflection and only even count of $T$ or $T^*$ is required. We also have $R^*RR^*$, $T^*RT^*$, \added{$R^*TT^*$ or $T^*TR^*$}. However, these four cases do not exist, since the reflection event at the outside of the surface can only happens at the upper hemisphere and vise versa. 

The next question is how to compute the contribution of the two new cases ($T^*T$ and $TT^*$) with refraction. \added{Here, we define K}.

Given the six cases of radiance change for $\rho_r^{o}$, we get the following equation to keep energy conservation: 
% \begin{equation}
% \begin{aligned}
% &\rho^o_r\left(\omega_{i}, \omega_{o}\right)= \frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)+1}\bigg(v^o_r\left(\omega_{i}, \omega_{o}\right)+\\
% &\int _{\Omega^+}\Big( v^o_r\left(\omega_{i}, -\omega\right)\rho^o_r \left(-\omega, \omega_{o}\right)+\rho^o_r\left(\omega_{i}, \omega\right) v^o_r\left(\omega, \omega_{o}\right)\Big) \mathrm{d}\omega \bigg)+\\
% &\int^\infty_{0}\bigg(\int _{\Omega^+}\Big(e^{-\tau|\Lambda\left(\omega_{i}\right)|}v^o_t\left(\omega_{i}, \omega\right)\rho^i_t\left(\left | \ln\left ( 1-e^{-\tau} \right )   \right | ,\infty,-\omega, -\omega_o\right)\\
% &+\rho^o_t\left(0,\tau,\omega_{i}, -\omega\right)v^i_t\left(\omega, -\omega_o\right)e^{-\left | \ln\left ( 1-e^{-\tau} \right )   \right |\Lambda\left(\omega_{o}\right)}\Big)\mathrm{d}\omega\bigg)\mathrm{d}\tau\\
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
&(\rho^o_r\left(\omega_{i}, \omega_{o}\right)-K_{TvT\rho}-K_{T\rho Tv})(|\Lambda\left(\omega_{i}\right)|+\Lambda\left(\omega_{o}\right))= \bigg(v^o_r\left(\omega_{i}, \omega_{o}\right)+\\
&\int _{\Omega^+}\Big( v^o_r\left(\omega_{i}, -\omega\right)\rho^o_r \left(-\omega, \omega_{o}\right)+\rho^o_r\left(\omega_{i}, \omega\right) v^o_r\left(\omega, \omega_{o}\right)\Big) \mathrm{d}\omega \bigg)\\
\end{aligned}
\end{equation}

%\begin{equation}
%\begin{aligned}
%&(\rho^o_t\left(\omega_{i}, \omega_{o}\right)-K_{Tv}-K_{TvR\rho}-K_{R\rho Tv})(|\Lambda\left(\omega_{i}\right)|-\Lambda\left(-\omega_{o}\right))=\\
%&\int _{\Omega^+}\Big( v^o_r\left(\omega_{i}, -\omega\right)\rho^o_t \left(-\omega, \omega_{o}\right)-\rho^o_t\left(\omega_{i}, -\omega\right) v^i_r\left(-\omega, \omega_{o}\right)\Big) \mathrm{d}\omega\\
%\end{aligned}
%\end{equation}

Similarly to the $\rho^o_r$, we also derive the formulation for other three cases, where the details are shown in the supplementary.

% \begin{equation}
% \begin{aligned}
% &\rho^i_r\left(\omega_{i}, \omega_{o}\right)= \frac{1}{\Lambda\left(-\omega_{i}\right)+\Lambda\left(\omega_{o}\right)+1}\bigg(v^i_r\left(\omega_{i}, \omega_{o}\right)+\\
% &\int _{\Omega^+}\Big( v^i_r\left(\omega_{i}, -\omega\right)\rho^i_r \left(-\omega, \omega_{o}\right)+\rho^i_r\left(\omega_{i}, \omega\right) v^i_r\left(\omega, \omega_{o}\right)\Big) \mathrm{d}\omega \bigg)+\\
% &\int^\infty_{0}\bigg(\int _{\Omega^+}\Big(e^{-\tau|\Lambda\left(\omega_{i}\right)|}v^i_t\left(\omega_{i}, \omega\right)\rho^o_t\left(\left | \ln\left ( 1-e^{-\tau} \right )   \right | ,\infty,-\omega, -\omega_o\right)\\
% &+\rho^i_t\left(0,\tau,\omega_{i}, -\omega\right)v^o_t\left(\omega, -\omega_o\right)e^{-\left | \ln\left ( 1-e^{-\tau} \right )   \right |\Lambda\left(\omega_{o}\right)}\Big)\mathrm{d}\omega \bigg)\mathrm{d}\tau\\
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &\rho^o_t\left(\tau_i,\tau_o,\omega_{i}, \omega_{o}\right)=\\
% &\int^{\max(\tau_i,\tau_o)}_{\min(\tau_i,\tau_o)}\bigg(e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^o_t\left(\omega_{i}, \omega_{o}\right)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}  \right |\right|\Lambda\left(-\omega_{o}\right)} \\
% &+\int _{\Omega^+}\Big(\rho^o_t\left (\tau_i,\tau, \omega_i,-\omega\right )v^i_r(\omega,-\omega_o)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\\
% &+e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^o_r(\omega_i,-\omega)\rho^o_t\left (\tau,\tau_o,-\omega, \omega_o \right ) \Big) \mathrm{d}\omega \bigg)\mathrm{d}\tau\\
% &+\int^\infty_{\tau_i} e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} v^o_t\left(\omega_{i}, \omega\right)\rho^i_r \left(-\omega, -\omega_{o}\right)\mathrm{d}\omega\\
% &+\int^{\tau_o}_0 e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} \rho^o_r\left(\omega_{i}, \omega\right) v^o_t\left(\omega, \omega_{o}\right)\mathrm{d}\omega\\
% &\rho^o_t\left(\omega_{i}, \omega_{o}\right)=\rho^o_t\left(0,\infty,\omega_{i}, \omega_{o}\right)\\
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &\rho^i_t\left(\tau_i,\tau_o,\omega_{i}, \omega_{o}\right)=\\
% &\int^{\max(\tau_i,\tau_o)}_{\min(\tau_i,\tau_o)}\bigg(e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^i_t\left(\omega_{i}, \omega_{o}\right)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}  \right |\right|\Lambda\left(-\omega_{o}\right)} \\
% &+\int _{\Omega^+}\Big(\rho^i_t\left (\tau_i,\tau, \omega_i,-\omega\right )v^o_r(\omega,-\omega_o)e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\\
% &+e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}v^i_r(\omega_i,-\omega)\rho^i_t\left (\tau,\tau_o,-\omega, \omega_o \right ) \Big) \mathrm{d}\omega \bigg)\mathrm{d}\tau\\
% &+\int^\infty_{\tau_i} e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} v^i_t\left(\omega_{i}, \omega\right)\rho^o_r \left(-\omega, -\omega_{o}\right)\mathrm{d}\omega\\
% &+\int^{\tau_o}_0 e^{-|\tau_i-\tau||\Lambda\left(\omega_{i}\right)|}e^{-\left|\ln\left | \frac{1-e^{-\tau}}{1-e^{-\tau_o}}\right |\right|\Lambda\left(-\omega_{o}\right)}\mathrm{d}\tau\\
% &\times \int _{\Omega^+} \rho^i_r\left(\omega_{i}, \omega\right) v^i_t\left(\omega, \omega_{o}\right)\mathrm{d}\omega\\
% &\rho^i_t\left(\omega_{i}, \omega_{o}\right)=\rho^i_t\left(0,\infty,\omega_{i}, \omega_{o}\right)\\
% \end{aligned}
% \end{equation}

In the reflection case, the shadowing-masking function for a light path can be easily obtained with the equation from the invariance principle. However, in the refraction case, we can not get the shadowing-masking function for a light path obviously, given the above four equations. We introduce the hypergeometric functions to solve these equations.

The hypergeometric functions are introduced by Gauss~\shortcite{gauss1812} and later extended to generalized hypergeometric functions by Pochhammer~\shortcite{pochhammer1870}, which are defined by infinite series:

%对此，我们并不能给出一个任意阶折射pathG的递归式。但我们仍然可以将其计算出来。

%我们首先需要引入一些数学工具。

%Gauss~\shortcite{gauss1812} 引入了超几何函数 ${_{2}F_{1}}$, Pochhammer~\shortcite{pochhammer1870} 将其推广为了广义超几何函数 ${_{p}F_{q}}$. 这些函数由无穷级数定义:
\begin{equation}
     \begin{aligned}
{_{p}F_{q}}\left(a_1,a_2,\cdots,a_p;b_1,b_2,\cdots,b_q,z\right)=\sum_{k=0}^{\infty}\frac{{\Tiny\displaystyle\prod_{i=1}^{p}} \frac{\Gamma \left ( a_i+k\right)}{\Gamma\left(a_i\right)}}{{\Tiny\displaystyle\prod_{j=1}^{q}}\frac{\Gamma \left ( b_j +k\right ) }{\Gamma \left ( b_j\right )}}\frac{z^k}{k!},
     \end{aligned}
    \label{eq:hypergeometric}
\end{equation}
 where $\Gamma$ is the Gamma function, and $(x-1)!$ is the analytic continuation. \added{We also need to define the other notations.}
 %$\Gamma$ 是伽马函数, 是 $(x-1)!$ 的解析延拓.

As we know the shadowing-masking function of a single bounce for the refractive surface is given by Pinel et al.~\shortcite{Pinel:05} using the Beta function:

%单次折射的pathG $S_{\mathrm{T}}$ 在\cite{Pinel:05}中已经给出, 其中用到了Beta函数:

\begin{equation}
     \begin{aligned}
    \mathrm{B}(a, b)=\int_{0}^{1} t^{a-1}(1-t)^{b-1} \mathrm{~d}t.
     \end{aligned}
    \label{eq:beta}
\end{equation}

Note that the Beta function and the Gamma function has the following relationship:
%这些函数有如下关系:
\begin{equation}
     \begin{aligned}
    \mathrm{B}(a, b)=\frac{\Gamma(a)\Gamma(b)}{\Gamma(a+b)}=\frac{1}{a}{_{2}F_{1}}(a,1-b;1+a,1).
     \end{aligned}
\end{equation}

However, we find that the Beta function can not solve the shadowing-masking function for more bounces. Thus, we propose a novel function, called \emph{generalized Beta functions}, which are defined as:
%当我们试图解决反射问题时，我们发现现有的数学工具已经无法满足我们的需要，我们得定义一些新函数，我们称为 \emph{generalized beta functions}:
\begin{equation}
     \begin{aligned}
 &\mathrm{B}^k(a_1,a_2,\cdots,a_k;b_1,b_2,\cdots,b_k)=\\ &\int_{\displaystyle [0,1]\times \prod_{m=1}^{k-1}[0,u_m ] }\prod_{n=1}^{k} u_n^{a_n-1}(1-u_n)^{b_n-1}\mathrm{~d}\mu\left(\overline{u}\right),
     \end{aligned}
    \label{eq:generalizedbeta}
\end{equation}
where $\mathrm{B}^1(a_1;b_1)=\mathrm{B}(a_1,b_1)$.

%这个函数有许多好的性质，例如对称性：
Note that this function is symmetric:
\begin{equation}
     \begin{aligned}
 &\mathrm{B}^k(a_1,a_2,\cdots,a_k;b_1,b_2,\cdots,b_k)=\\
 &\mathrm{B}^k(b_k,b_{k-1},\cdots,b_1;a_k,a_{k-1},\cdots,a_1)
     \end{aligned}
\end{equation}
\added{Note that we can not prove this symmetric property, but we check the numerical values.}

With the generalized Beta function, we finally derive the shadowing-masking function for a path with refraction. 
%We can derive some equations for at least three bounces. For more bounces, 
%定义了这些之后，我们就可以表示出带有折射的pathG。

%以下是包含折射的2次散射的所有pathG：
The shadowing-masking function for a path with refraction-reflection is: 

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TR}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=\\
&\begin{cases}
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{1}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|)-\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{2}\right)|-|\Lambda\left(\mathbf{d}_{1}\right)|}, \text { if } \mathbf{d}_{1} . z<0 \\
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{2}\right)|+\Lambda\left(\mathbf{d}_{1}\right)}, \text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}

The reflection-refraction case is symmetric to the above equation, thus we show it in the supplementary. Then we show the equation for the refraction-refraction case:

% \begin{equation}
%      \begin{aligned}
% &S_{\mathrm{RT}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=\\
% &\begin{cases}
% \frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{1}\right)|,|\Lambda\left(\mathbf{d}_{2}\right)|)-\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{0}\right)|-|\Lambda\left(\mathbf{d}_{1}\right)|}, \text { if } \mathbf{d}_{1} . z<0 \\
% \frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{2}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{1}\right)}, \text { if } \mathbf{d}_{1} . z>0
% \end{cases}
%      \end{aligned}
% \end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TT}}\left(\mathbf{d}_{0}, \mathbf{d}_{1}, \mathbf{d}_{2}\right)=\\
&\begin{cases}
\mathrm{B}^2(|\Lambda\left(\mathbf{d}_{0}\right)|,\Lambda\left(\mathbf{d}_{2}\right)+1;-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1), \text { if } \mathbf{d}_{1} . z<0 \\
\mathrm{B}^2(\Lambda\left(\mathbf{d}_{2}\right)+1,|\Lambda\left(\mathbf{d}_{0}\right)|;\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right)), \text { if } \mathbf{d}_{1} . z>0
\end{cases}
     \end{aligned}
\end{equation}

%3次：

For three bounces, we show the TRR (RRT), RTR, TTR (RTT), TRT and TTT.

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TRR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{2}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}}{\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)},\\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{2}\right)\right|+\Lambda\left(\mathbf{d}_{1}\right)}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{3}\right)\right|+\Lambda\left(\mathbf{d}_{1}\right)}}{\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{3}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{(|\Lambda\left(\mathbf{d}_{3}\right)|+\Lambda\left(\mathbf{d}_{2}\right))(|\Lambda\left(\mathbf{d}_{3}\right)|+\Lambda\left(\mathbf{d}_{1}\right))}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{RTR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}}{\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)}, \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left(\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|\right)\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|+\Lambda\left(\mathbf{d}_{2}\right)\right)}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|\right)\left(\left|\Lambda\left(\mathbf{d}_{0}\right)\right|+\Lambda\left(\mathbf{d}_{1}\right)\right)}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{3}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{(|\Lambda\left(\mathbf{d}_{3}\right)|+\Lambda\left(\mathbf{d}_{2}\right))(|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{1}\right))}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

% \begin{equation}
%      \begin{aligned}
% &S_{\mathrm{RRT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
% &\begin{cases}
% \frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{1}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{2}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)-\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{2}\right)\right|}}{\left(\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|\right)}, \\
% \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
% \frac{\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\left|\Lambda\left(\mathbf{d}_{3}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{1}\right)\right|+\Lambda\left(\mathbf{d}_{2}\right)}-\frac{\mathrm{B}\left(\left|\Lambda\left(\mathbf{d}_{3}\right)\right|,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|+\Lambda\left(\mathbf{d}_{2}\right)}}{\left|\Lambda\left(\mathbf{d}_{0}\right)\right|-\left|\Lambda\left(\mathbf{d}_{1}\right)\right|}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
% \frac{\mathrm{B}(|\Lambda\left(\mathbf{d}_{3}\right)|,|\Lambda\left(\mathbf{d}_{0}\right)|) }{(|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{2}\right))(|\Lambda\left(\mathbf{d}_{0}\right)|+\Lambda\left(\mathbf{d}_{1}\right))}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
% \end{cases}
%      \end{aligned}
% \end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TTR}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)\\
-\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
\frac{\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{3}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{2}\right)+1\right)\\
-\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TRT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{1}\right)+1,-\Lambda\left(\mathbf{d}_{1}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)\\
-\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right);\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)\\
+\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\frac{1}{\Lambda\left(\mathbf{d}_{1}\right)-\Lambda\left(\mathbf{d}_{2}\right)}(\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)\\
-\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{1}\right),\Lambda\left(\mathbf{d}_{1}\right)+1;\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

% \begin{equation}
%      \begin{aligned}
% &S_{\mathrm{RTT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
% &\begin{cases}
% \frac{1}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}(\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{1}\right)\right|\right)\\
% -\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)),\\
% \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
% \frac{\mathrm{B}^2\left(\Lambda\left(\mathbf{d}_{2}\right)+1,-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{3}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|\right)}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}, \text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
% \frac{1}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}(\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{1}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)\\
% -\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)), \\
% \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
% \frac{\mathrm{B}^2\left(-\Lambda\left(\mathbf{d}_{2}\right),\Lambda\left(\mathbf{d}_{2}\right)+1,\left|\Lambda\left(\mathbf{d}_{0}\right)\right|,\Lambda\left(\mathbf{d}_{3}\right)+1\right)}{\Lambda\left(\mathbf{d}_{1}\right)+\left|\Lambda\left(\mathbf{d}_{0}\right)\right|}, \text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
% \end{cases}
%      \end{aligned}
% \end{equation}

\begin{equation}
     \begin{aligned}
&S_{\mathrm{TTT}}\left(\mathbf{d}_{0}, \cdots, \mathbf{d}_{3}\right)=\\
&\begin{cases}
\mathrm{B}^3(|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2);-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z<0\\
\mathrm{B}(|\Lambda(\mathbf{d}_0)|,-\Lambda(\mathbf{d}_1))\mathrm{B}^2(\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|;\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2))\\
-\mathrm{B}^3(-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|;|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2)), \\
\text { if } \mathbf{d}_{1} . z<0 \text { and } \mathbf{d}_{2} . z>0\\
\mathrm{B}(|\Lambda(\mathbf{d}_0)|,-\Lambda(\mathbf{d}_1))\mathrm{B}^2(\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2);\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|)\\
-\mathrm{B}^3(|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2);-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z<0\\
\mathrm{B}^3(-\Lambda(\mathbf{d}_1),\Lambda(\mathbf{d}_1)+1,|\Lambda(\mathbf{d}_3)|;|\Lambda(\mathbf{d}_0)|,\Lambda(\mathbf{d}_2)+1,-\Lambda(\mathbf{d}_2)), \\
\text { if } \mathbf{d}_{1} . z>0 \text { and } \mathbf{d}_{2} . z>0\\
\end{cases}
     \end{aligned}
\end{equation}

The equation for more bounces can be similarly derived. For a light path with $n$ refractive interactions can be represented with a n-order generalized Beta function.  

The next question is how to solve these generalized Beta function. For the two-order generalized Beta function, we have:
%对于二次的广义beta函数，我们可以得到：

\begin{equation}
\begin{aligned}
&\mathrm{B}^2(a_1,a_2;b_1,b_2)  \\
=& \frac{1}{a_2}\mathrm{B}\left ( a_1+a_2,b_1 \right ) {_{3}F_{2}}\left ( a_2,1-b_2,a_1+a_2;a_2+1,a_1+a_2+b_1,1 \right ). \\
\end{aligned}
\end{equation}

However, for higher orders, the generalized Beta function can not be solved analytically bu the current mathematical tool, and we leave this problem for the future work. 

To summarize, we can provide the formulation of the refractive surface with any bounces, but the current mathematical tool can only solve at most two refractive interactions. Therefore, we use our proposed model for all the reflection case with any bounce, all the two-bounce cases and all the three-bounce cases except TTT. We leave the other cases with the random walk solution, similar to Heitz et al.~\shortcite{heitz2016}.

% \begin{equation}
% \begin{aligned}
% &\mathrm{B}^2(a_1,a_2;b_1,b_2)  \\
% =& \int_{0}^{1} \int_{0}^{\mathcal{U}_1} \mathcal{U}_1^{a_1-1}(1-\mathcal{U}_1)^{b_1-1}\mathcal{U}_2^{a_2-1}(1-\mathcal{U}_2)^{b_2-1}\mathrm{~d}\mathcal{U}_2\mathrm{d}\mathcal{U}_1 \\
% =& \int_{0}^{1} \mathcal{U}_1^{a_1-1}(1-\mathcal{U}_1)^{b_1-1}\mathrm{B}(\mathcal{U}_1 ;a_2,b_2) \mathrm{~d}\mathcal{U}_1 \\
% =&\frac{1}{a_2}\int_{0}^{1} \mathcal{U}_1^{a_1+a_2-1}(1-\mathcal{U}_1)^{b_1-1}{_{2}F_{1}}(a_2,1-b_2;1+a_2,\mathcal{U}_1) \mathrm{~d}\mathcal{U}_1 \\
% =&\frac{1}{a_2}\sum_{k=0}^{\infty}\left ( \frac{\frac{\Gamma \left ( a_2+k\right)}{\Gamma\left(a_2\right)}\frac{\Gamma \left ( 1-b_2+k\right)}{\Gamma\left(1-b_2\right)}}{\frac{\Gamma \left ( a_2+1+k\right ) }{\Gamma \left ( a_2+1\right )}k!}\int_{0}^{1} \mathcal{U}_1^{a_1+a_2+k-1}(1-\mathcal{U}_1)^{b_1-1} \mathrm{~d}\mathcal{U}_1 \right ) \\
% =&\frac{1}{a_2}\sum_{k=0}^{\infty}\left ( \frac{\frac{\Gamma \left ( a_2+k\right)}{\Gamma\left(a_2\right)}\frac{\Gamma \left ( 1-b_2+k\right)}{\Gamma\left(1-b_2\right)}}{\frac{\Gamma \left ( a_2+1+k\right ) }{\Gamma \left ( a_2+1\right )}k!}\frac{\Gamma \left ( a_1+a_2+k\right ) \Gamma \left ( b_1\right )}{\Gamma \left ( a_1+a_2+b_1+k\right )} \right ) \\
% =&\frac{1}{a_2}\sum_{k=0}^{\infty}\left ( \frac{\frac{\Gamma \left ( a_2+k\right)}{\Gamma\left(a_2\right)}\frac{\Gamma \left ( 1-b_2+k\right)}{\Gamma\left(1-b_2\right)}}{\frac{\Gamma \left ( a_2+1+k\right ) }{\Gamma \left ( a_2+1\right )}k!}\frac{\frac{\Gamma \left ( a_1+a_2+k\right )}{\Gamma \left ( a_1+a_2\right )}}{\frac{\Gamma \left ( a_1+a_2+b_1+k\right )}{\Gamma \left ( a_1+a_2+b_1\right )} } \right )\frac{\Gamma \left ( a_1+a_2\right )\Gamma \left ( b_1\right )}{\Gamma \left ( a_1+a_2+b_1\right )}  \\
% =& \frac{1}{a_2}\mathrm{B}\left ( a_1+a_2,b_1 \right ) {_{3}F_{2}}\left ( a_2,1-b_2,a_1+a_2;a_2+1,a_1+a_2+b_1,1 \right ) \\
% \end{aligned}
% \end{equation}

%但可惜的是，三次及以上的广义beta函数并不能被现有的数学工具解析的表示，我们只能把这个问题留给数学界。

%我们可以表明的是，含有n次折射过程的pathG，其中必含有n次的广义beta函数，所以我们目前只能解析的计算所有纯粹反射，带折射的所有2次的情况及除了 TTT 以外的所有3次的情况，对于其他的情况，我们回退到随机游走进行计算。


